Approximating the Minimal Lookahead Needed to Win Infinite Games

We present an exponential-time algorithm approximating the minimal lookahead necessary to win an $\omega$-regular delay game.

==> content/frontmatter.tex <==
\begin{frontmatter}

\title{Approximating the Minimal Lookahead\\ Needed to Win Infinite Games}
\author{Martin Zimmermann}

\address{University of Liverpool \footnote{Current affiliation: Aalborg University, Aalborg, Denmark.}}

\begin{abstract}
We present an exponential-time algorithm approximating the minimal lookahead necessary to win an $\omega$-regular delay game. \end{abstract}

\begin{keyword}
Delay Games \sep Approximation Algorithm \sep Infinite Games
\end{keyword}

\end{frontmatter}
